A template method for measuring the iron spectrum in cosmic rays with Cherenkov telescopes

The energy-dependent abundance of elements in cosmic rays plays an important role in understanding their acceleration and propagation. Most current results are obtained either from direct measurements by balloon- or satellite-borne detectors, or from indirect measurements by air shower detector arrays on the Earth's surface. Imaging Atmospheric Cherenkov Telescopes (IACTs), used primarily for $\gamma$-ray astronomy, can also be used for cosmic-ray physics. They are able to measure Cherenkov light emitted both by heavy nuclei and by secondary particles produced in air showers, and are thus sensitive to the charge and energy of cosmic ray particles with energies of tens to hundreds of TeV. A template-based method, which can be used to reconstruct the charge and energy of primary particles simultaneously from images taken by IACTs, will be introduced. Heavy nuclei, such as iron, can be separated from lighter cosmic rays with this method, and thus the abundance and spectrum of these nuclei can be measured in the range of tens to hundreds of TeV.

==> definitions.tex <==

\usepackage{graphicx}
\usepackage[square,sort&compress]{natbib}
\usepackage{overpic}
\usepackage{amsfonts, amsmath, amsthm, amssymb} % For math fonts, symbols and environments
\usepackage{wasysym}
\usepackage{url}
\usepackage[amssymb,textstyle]{SIunits}
\usepackage{booktabs}
\usepackage{afterpage}

\addunit{\GeV}{\giga\electronvolt}
\addunit{\TeV}{\tera\electronvolt}
\addunit{\eV}{\electronvolt}
\addunit{\smm}{\square\metre\usk\second}
\addunit{\smmr}{\rpsquare\metre\usk\reciprocal\second}

\newcommand{\e}[1]{\cdot\power{10}{#1}}

\usepackage{setspace}
\usepackage[svgnames]{xcolor} % Specify colors by their 'svgnames', for a full list of all colors available see here: http://www.latextemplates.com/svgnames-colors

\definecolor{desyCyan}{RGB}{0,166,235}
\definecolor{desyOrange}{RGB}{242,142,0}
\definecolor{desyGrau}{RGB}{119,119,119}
\definecolor{desyHell}{RGB}{119,119,119}

%\usepackage[font=small,labelfont=bf]{caption} % Required for specifying captions to tables and figures
\usepackage{wrapfig} % Allows wrapping text around tables and figures

\newcommand{\desyDot}{{\color{desyOrange}\textrm{.}}}

